Learning Coupled Policies for Simultaneous Machine Translation using Imitation Learning

We present a novel approach to efficiently learn a simultaneous translation model with coupled programmer-interpreter policies. First, wepresent an algorithmic oracle to produce oracle READ/WRITE actions for training bilingual sentence-pairs using the notion of word alignments. This oracle actions are designed to capture enough information from the partial input before writing the output. Next, we perform a coupled scheduled sampling to effectively mitigate the exposure bias when learning both policies jointly with imitation learning. Experiments on six language-pairs show our method outperforms strong baselines in terms of translation quality while keeping the translation delay low.

==> tables/table_ss_rate.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|cc|cc|cc|cc|cc|}
    \hline
     NMT \texttt{\textbackslash} Agent
     & \multicolumn{2}{c|}{0.05} 
     & \multicolumn{2}{c|}{0.05} 
     & \multicolumn{2}{c|}{0.15} 
     & \multicolumn{2}{c|}{0.25} 
     & \multicolumn{2}{c|}{0.35} 
     \\ \hline \hline
   0 & 17.53 & 5.05 & 20.40 & 4.07 & 22.37 & 4.11 & 23.83 & 4.38 & 22.23 & 4.39\\
0.05 & 15.57 & 5.43 & 20.72 & 4.15 & 22.37 & 4.02 & 23.04 & 4.20 & 23.18 & 4.38\\
0.15 & 14.64 & 5.02 & 21.82 & 4.20 & 24.12 & 3.98 & 24.33 & 4.03 & 24.04 & 4.04\\
0.25 & 16.72 & 5.37 & 21.22 & 3.98 & 23.35 & 3.90 & 21.95 & 3.83 & 22.64 & 4.03\\
0.35 & 17.01 & 5.73 & 19.86 & 3.96 & 20.95 & 3.76 & 23.50 & 3.94 & 22.56 & 4.00\\
\hline
    \end{tabular}
    \caption{Column: ss on agent, Row: ss on model}
    \label{tab:my_label}
\end{table*}
